Generation of fresh and pure random numbers for loophole-free Bell tests

We demonstrate extraction of randomness from spontaneous-emission events less than 36 ns in the past, giving output bits with excess predictability below $10^{-5}$ and strong metrological randomness assurances. This randomness generation strategy satisfies the stringent requirements for unpredictable basis choices in current "loophole-free Bell tests" of local realism [Hensen et al., Nature (London) 526, 682 (2015); Giustina et al., Phys. Rev. Lett. 115, 250401 (2015); Shalm et al., Phys. Rev. Lett. 115, 250402 (2015)].

==> NoSOM.tex <==
\citation{Henry:1982dv}
\citation{AgrawalJQE1990,ScullyZubairy1997}
\citation{AbellanOE2014,Yuan:2014co}
\citation{RauchAIAAJ1965,GelbBook1974}
\citation{AgrawalJQE1990,ScullyZubairy1997}
\citation{EinsteinDPG1916}
\citation{KoflerARX2014b,LarssonJPA2014}
\citation{LEcuyerACM2007}
\citation{RukhinNIST2010tech}
\citation{BrownWEB2004b}
\citation{RukhinNIST2010tech}
\citation{JacobsenMaster2014}
\bibstyle{apsrev4-1no-url}
\bibdata{SOMNotes,./freshqrng}

